A survey of computational frameworks for solving the acoustic inverse problem in three-dimensional photoacoustic computed tomography

Photoacoustic computed tomography (PACT), also known as optoacoustic tomography, is an emerging imaging technique that holds great promise for biomedical imaging. PACT is a hybrid imaging method that can exploit the strong endogenous contrast of optical methods along with the high spatial resolution of ultrasound methods. In its canonical form that is addressed in this article, PACT seeks to estimate the photoacoustically-induced initial pressure distribution within the object. Image reconstruction methods are employed to solve the acoustic inverse problem associated with the image formation process. When an idealized imaging scenario is considered, analytic solutions to the PACT inverse problem are available; however, in practice, numerous challenges exist that are more readily addressed within an optimization-based, or iterative, image reconstruction framework. In this article, the PACT image reconstruction problem is reviewed within the context of modern optimization-based image reconstruction methodologies. Imaging models that relate the measured photoacoustic wavefields to the sought-after object function are described in their continuous and discrete forms. The basic principles of optimization-based image reconstruction from discrete PACT measurement data are presented, which includes a review of methods for modeling the PACT measurement system response and other important physical factors. Non-conventional formulations of the PACT image reconstruction problem, in which acoustic parameters of the medium are concurrently estimated along with the PACT image, are also introduced and reviewed.

==> section3/section3c-old.tex <==
\subsection{D-D forward models for use with heterogeneous acoustic media}
\label{subsec:section3c}
\if 0
A digital imaging system is accurately described  by a continous-to-discrete imaging model, which is typically approximated in practice by a discrete-to-discrete(D-D) imaging model to facilitate the application of numerical image reconstruction algorithms. 
\fi 
In this section, a D-D imaging model for photoacoustic imaging in lossy, heterogeneous media is presented. The developed D-D imaging model can then be subsequently employed in the formulation of iterative algorithms described in the later sections. 

The construction of a D-D imaging model for lossy, heterogeneous media requires the introduction of finite-dimensional approximations of the object function $p_0(\mathbf{r})$ as well as the medium parameters such as $c(\mathbf{r}), \rho_0(\mathbf{r})$ and $\alpha(\mathbf{r})$. For photoacoustic imaging in heterogeneous media, the choice of finite-dimensional representation of the object and medium parameters is dictated by the numerical method employed to solve the coupled first order differential equations described in Eqn.~\eref{eq:2a_loss}. Most methods for solving the numerical solution to the acoustic wave equation in lossy heterogeneous media fall into one of three major categories: finite difference (FD) methods, finite element(FE) methods and spectral methods. We will briefly discuss the salient features of each of these methods and its applications to photoacoustic imaging.

\subsubsection{Finite element Methods}
The finite element (FE) method is a popular and powerful method for calculating numerical solutions to partial differential equations due to its computational efficiency, ability to accommodate tissue heterogeneity, geometric irregularities as well as to allow complex boundary conditions and source representations. In the FE method, the solution is represented by a linear combination of N-dimensional basis functions defined on the computational domain, and the unknown amplitudes of these basis functions are estimated to find the solution. The flexibilities in the choice of the basis functions allows domains and heterogeneities of arbitrary shape to be accurately represented. As the FE method can model arbitrary geometries, encoding the FE is not as straightforward as the FD or k-space methods discussed in the following sections. Although, commercial packages are available to ease the burden, FE methods have not gained traction in the photoacoustic community as they are not as straightforward to implement. In addition, when solving wave equations with the FE method, about 10 nodes per wavelength are required to represent the wavefield accurately. As a consequence, FE becomes cumbersome and slow for modelling large scale, high frequency applications of PACT. Although FE methods are not well suited for high frequency applications of PACT, they have been widely employed to compute low frequency solutions of PA equation~\cite{jiang2006spatially,yuan2007three,yao2009finite,yao2011enhancing}. 

\subsubsection{Finite Difference Methods}
 Another technique that is in widespread use for finding numerical solutions to partial differential equations is the finite difference (FD) method. In the FD method, the derivatives of the partial differential equation are approximated by the method of differences, converting the set of partial differential equations into a set of difference equations that can be solved numerically. As the FD models are less flexible than FE models, the FD method is not as adept at representing complex geometries, heterogeneities and boundary conditions accurately. Even though the FD method is not as flexible as FE methods, it has gained popularity in numerical modeling as it is conceptually simple and straightforward to implement. Similar to FE methods, the FD methods also suffer from the same stringent spatial sampling requirements. Thus, FD methods become intractable for modelling large scale, high-frequency applications of PACT. Even though
 FD methods are cumbersome and slow for large scale applications of PACT,they have been widely employed for modeling PA wave propagation due to their conceptual simplicity and  straightforward implementation~\cite{huang2005simulations,mast1997simulation,sheu2008simulations,burgholzer2007exact}. 
 
 For time domain problems in PACT, it is common practice to approximate the time derivative using a FD approximation. Hence, the spatial part of the solution is solved using FD or FE methods, while the temporal propagation is performed using the FD method. Hence, to avoid numerical dispersion in the temporal domain the time steps in both the FD and FE methods have to be small, further reducing the efficiency of both FE and FD time domain models.  
 
\subsubsection{Spectral methods}
The FD and FE methods are also known as local methods as the wave propagation equations are solved at each point based only on conditions at neighboring points. In contrast, spectral methods such as the k-space method and the pseudospectral apporach, are global because information from the entire wavefield is employed to solve the wave propagation at each point. Due to its global nature, spectral methods can be more accurate than local methods. As the spectral methods leverage global information to solve the wave propagation, they allow compuation to be performed on coarser grid while maintaining the same accuracy~\cite{gottlieb1977numerical}. As opposed to FD or FE methods that require grid spacings on the order 10 points per minimum wavelength, the spectral methods, in theory, only require 2 points per minimum wavelength. Due to such relaxed spatial sampling constraints, spectral methods are well suited for large-scale, high frequency PA wave solvers. 

The most popular spectral method that is well-suited for solving the acoustic wave equation in Eqn.~\eref{eq:2a_loss} is based on the Fourier transform  and is referred to as the pseudospectral method~\cite{kreiss1972comparison,witte1989pseudospectral,liu1998pseudospectral}. In the classical pseudospectral time-domain (PSTD) method, the spatial derivatives are estimated globally through the use of Fourier transformation and the temporal derivatives are computed using the FD scheme~\cite{wojcik1997pseudospectral}. A spatial derivative operator in the classical pseudospectral scheme can be written as 
\begin{align}
\frac{\partial[\cdot]}{\partial x} = \mathcal{F}^{-1}\{i k_x \mathcal{F}\{[\cdot]\}\},
\end{align}
where $\mathcal{F}, \mathcal{F}^{-1}$ represent the Fourier and inverse Fourier transformations and $k_x$ represents the wave number along x-axis. The classical PSTD methods require the temporal step size to be very small, which reduces its computational efficiency. The k-space family of methods can overcome this problem by utilizing explicit temporal propagators related to the Green's function for wave propagation in \textit{k-t} (spatial frequency and time) space. Thus, the k-space PSTD method for solving wave equation allows for the use of much larger time steps without sacrificing accuracy and stability~\cite{mast2001k,tabei2002k}. In the k-space PSTD method, the spatial derivative operator is computed by use of a temporal propagator as 
\begin{align}\label{eq:3c_propagator}
\frac{\partial[\cdot]}{\partial x} = \mathcal{F}^{-1}\{i k_x sinc\Big(\frac{c_{max}k\Delta t}{2}\Big) \mathcal{F}\{[\cdot]\}\},
\end{align}
where $c_{max}$ is the maximum sound speed of the heterogeneous medium, $k$ is the total wave number, and $\Delta t $ is the time interval. Using the spatial derivative operator in Eqn.~\eref{eq:3c_propagator}, the time derivative can be stably calculated via the FD scheme in the k-space PSTD method with large time steps. Several benchmark studies~\cite{mast2001k,tabei2002k,liu1995generalization,bojarski1982k} have been conducted that illustrate the increased accuracy and stability of the k-space PSTD method compared with the time domain FD method as well as the classical PSTD method. In addition to being efficient by virtue of the reduced per-wavelength requirement, the use of larger time steps made possible by the k-space propagator and the use of FFT to calculate gradients in the k-space, the k-space PSTD is also extremely straightforward to encode. Hence, in view of these advantages, the k-space PSTD method has become widely employed as a standard numerical tool for modeling PA wave propagation~\cite{treeby2010photoacoustic,cox2007k,mast2001k}.  

The salient features of the k-space PSTD that underlie the discrete PACT imaging model are described below. The approximate finite-dimensional approximations of the object function $p_0(\mathbf{r})$ as well as the medium parameters $c(\mathbf{r}), \rho_0(\mathbf{r})$ and $\alpha(\mathbf{r})$ are constructed by sampling these quantities on a Cartesian grid. If $\{\phi_n^{\rm int}(\mathbf{r})\}_{n = 0}^{N-1}$ denote the set of 3D cartesian expansion functions defined in Eqn.~\eref{eq:3b_interpolation_expansion}, then we can approximate the initial pressure distribution $p_0(\mathbf{r})$ as a finite dimensional vector $\boldsymbol{\theta} \in \mathbb{R}^{N \times 1}$.

% defined as 
%\begin{align}\label{eq:3c_Fin}
%\phi_n(\mathbf{r}) = \begin{cases}
%1,&\ \ \ \text{if } |x - x_n|\leq \epsilon \text{ and } |y - y_n| \leq \epsilon \text{ and } |z - z_n| \leq \epsilon \\
%0,&\ \ \ \text{otherwise}
%\end{cases},
%\end{align}
%where $\mathbf{r} = (x,y,z)^T$ and $\mathbf{r}_n = (x_n,y_n,z_n)^T$ 
To ensure the stability of the k-space PSTD method, the material properties such as the speed of sound $c(\mathbf{r})$, the ambient density $\rho_0(\mathbf{r})$, the absorption coefficient $\alpha(\mathbf{r})$, and the wavefield parameters such as pressure $p(\mathbf{r}, t)$,  particle velocity $\mathbf{u}(\mathbf{r}, t)$, accoustic density $\rho(\mathbf{r},t)$ are sampled at different points of the staggered cartesian grids~\cite{treeby2010k}. Furthermore, the wavefield parameters such as the pressure, particle velocity and acoustic density are staggered temporally. Thus, to obtain finite-dimensional representations of the medium parameters and the wavefield parameters for use in a D-D imaging model, different expansion functions needs to be employed. For convenience, we will skip over some of these details and assume that the finite dimensional approximations of the continuous variables can be readily obtained. 


Let $\mathbf{u}^i_k \in \mathbb{R}^{N \times 1}$, $\boldsymbol{\rho}^i_k \in \mathbb{R}^{N \times 1}$ represent the discrete approximations of the vector-valued particle velocity and acoustic density over the whole 3D cartesian grid at $k^{th}$ time step along the $i^{th}$ direction and $\mathbf{p}_k \in \mathbb{R}^{N \times 1}$ represent the acoustic pressure along the whole grid at the $k^{th}$ time step. We can model the propagation of the wavefield parameters as each time step as 
\begin{align}
\mathbf{v}_{k+1} = \mathbf{W'}\mathbf{v}_k,
\end{align}
where $\mathbf{v}_k = (\mathbf{u}_k^1, \mathbf{u}_k^2, \mathbf{u}_k^3, \boldsymbol{\rho}_k^1, \boldsymbol{\rho}_k^2, \boldsymbol{\rho}_k^3, \mathbf{p}_k)^T$ is a $7N \times 1$ vector containing all the wavefield variables at the time step $k\Delta t$. The matrix $\mathbf{W'} \in \mathbb{R}^{7N \times 7N}$ is called the propagator matrix and can be readily derived from Eqn.~\eref{eq:2a_loss}~\cite{huang2013full}. Given a time propagator matrix that models the update of all the field parameters at each time step, we can model the imaging process in PACT as the propagation of the wavefield parameters forward in time from $t = 0$ to $t = (K-1)\Delta t$ 
\begin{align}\label{eq:3c_Prop}
\begin{bmatrix}\mathbf{v}_0, \mathbf{v}_1, \cdots, \mathbf{v}_{K-1}
\end{bmatrix}^T = \mathbf{T}_{K-1} \cdot \mathbf{T}_{K-2} \cdots \mathbf{T}_1
\begin{bmatrix}
\mathbf{v}_0,\mathbf{0}_{7N \times 1},\cdots,\mathbf{0}_{7N \times 1}
\end{bmatrix}^T.
\end{align}
The temporal matrix $\mathbf{T}_k (k = 1,\cdots, K-1) \in \mathbb{R}^{7NK \times 7NK}$ can be readily derived from Eqn~\eref{eq:2a_loss}~\cite{huang2013full}.
\if 0
Here, the temporal matrix $\mathbf{T}_k (k = 1,\cdots, K-1) \in \mathbb{R}^{7NK \times 7NK}$ can be defined in terms of $\mathbf{W'}$ as
\begin{align}
\mathbf{T}_k \equiv 
\begin{bmatrix}
&\mathbf{I}_{7N \times 7N} &\cdots &\mathbf{0}_{7N \times 7N}  &\\
&\vdots &\ddots &\vdots &\mathbf{0}_{(k+1)\cdot 7N \times (K-k)\cdot 7N}\\
&\mathbf{0}_{7N \times 7N} &\cdots &\mathbf{I}_{7N \times 7N} &\  \\
&\mathbf{0}_{7N \times 7N} &\cdots &\mathbf{W'} &\  \\
&\mathbf{0}_{(K-k-1)\cdot 7N \times k\cdot 7N} &\  &\  &\mathbf{0}_{(K-k-1)\cdot 7N \times (K-k)\cdot 7N}
\end{bmatrix},
\end{align} 
\
with $\mathbf{W'}$ residing between $(7N(k-1) + 1)^{th}$ to $7Nk^{th}$ columns and the $(7Nk + 1)^{th}$ to $7N(k +1)^{th}$ rows of $\mathbf{T}_k$.
\fi
From the initial conditions defined in Eqn.~\eref{eq:2a_loss}, the vector $(\mathbf{v}_0, \mathbf{0}_{7N\times 1}, \cdots, \mathbf{0}_{7N \times 1})^T$ can be computed from the initial pressure distribution $\boldsymbol{\theta}$ as 
\begin{align}\label{eq:3c_Init}
\begin{bmatrix}
\mathbf{v}_0, \mathbf{0}_{7N \times 1}, \cdots, \mathbf{0}_{7N \times 1}
\end{bmatrix}^T = \mathbf{T}_0 \boldsymbol{\theta},
\end{align}
where $\mathbf{T}_0 \in \mathbb{R}^{7N \times N}$ maps the initial pressure distribution to the initial value of the wavefield variables at time $t = 0$~\cite{huang2013full}.

In general, the transducer locations $\mathbf{r}_q^{\prime}$ at which the pressure $\tilde{\mathbf{p}}$ are recorded will not coincide with the vertices of the 3D Cartesian grid at which the propagated wavefields are computed. The pressure at the transducer locations can be related to the computed field quantities via an interpolation operation defined as 
\begin{align}\label{eq:3c_Interp}
\tilde{\mathbf{p}} = \mathbf{M}\begin{bmatrix}
\mathbf{v}_0, \mathbf{v}_1, \cdots, \mathbf{v}_{K-1}
\end{bmatrix}^T,
\end{align}
where $\mathbf{M} \in \mathbb{R}^{QPK \times 7NM}$. The choice of the interpolation operation is a design parameter that will constrain the construction of the matrix $\mathbf{M}$. Some of the most commonly employed interpolation strategies include trilinear interpolation or Delaunay triangulation-based interpolation~\cite{lee1980two}. 

By use of Eqns.~\eref{eq:3c_Init},~\eref{eq:3c_Prop} and~\eref{eq:3c_Interp}, one obtains
\begin{align}\label{eq:3c_Imageeqn}
\tilde{\mathbf{p}} = \mathbf{M}\mathbf{T}_{K-1}\cdots \mathbf{T}_1 \mathbf{T}_0 \boldsymbol{\theta}.
\end{align}
The explicit form of the system matrix $\mathbf{H}_{PS} \in \mathbb{R}^{QPK \times N}$, that describes the propagation of PA waves based on Eqn.~\eref{eq:2a_loss} can be written as
\begin{align}\label{eq:3c_HPS}
\mathbf{H}_{PS} = \mathbf{M}\mathbf{T}_{K-1}\cdots \mathbf{T}_1 \mathbf{T}_0.
\end{align}
Here, the subscript $PS$ stands for the fact that the D-D imaging model is computed using the k-space PSTD method. 


==> section3/section3d_iii.tex <==
\subsubsection{Heterogenous case: See Chao's TMI paper, cite Cox}
The system matrix defined in Eqns.~\eref{eq:3c_Imageeqn} and~\eref{eq:3c_HPS} did not incorporate the transducer's impulse response. An important feature of the proposed discrete imaging model in Eqns.~\eref{eq:3c_Imageeqn} is that the transducer's impulse responses, including the spatial impulse response (SIR) and the acousto-electrical impulse response (EIR), can be readily incorporated into the system matrix. 

The SIR of the transducer describes the averaging effect over the surface of the transducer~\cite{harris1981review,andreev2002detection,wang2011imaging}. It can be written as
\begin{align}
\tilde{p}^{SIR}(\mathbf{r}_q^{\prime}, k \Delta t) = \frac{\int_{S(\mathbf{r}_q)} dS(\mathbf{r}_q) \tilde{p}(\mathbf{r}_q, k \Delta t)}{S(\mathbf{r}_q^{\prime})},
\end{align}
where $\tilde{p}^{SIR}(\mathbf{r}_q^{\prime}, k\Delta t)$ is the pressure at time $t = k \Delta t$ averaged over the the surface of the $q^{th}$ transducer centered at $\mathbf{r}_q^{\prime}$. In order to incorporate the SIR into the proposed discrete imaging model we need to divide the transducer surface into $P$ small patches each with an equal area of $\Delta S$. The value of $P$ should be chosen such that the area $\Delta S$ is much less than the acoustic wavelength. Given this constraint, the integral in Eqn.~\eref{eq:3diii_SIRc} can be approximated numerically by
\begin{align}\label{eq:3diii_SIRc}
\tilde{p}^{SIR}(\mathbf{r}_q^{\prime}, k \Delta t) \approx \sum_{p = 1}^P \tilde{p}(\mathbf{r}_q^p, k \Delta t) \frac{\Delta S}{S(\mathbf{r}_q^p)}
\end{align}
Recall that the measured pressure data $\tilde{\mathbf{p}} \in \mathbb{R}^{QPK \times 1}$ is defined for $QP$ number of point transducers. By definition we know,
\begin{align}
\tilde{\mathbf{p}} \equiv \begin{bmatrix}
\tilde{\mathbf{p}}_0, \cdots, \tilde{\mathbf{p}}_{K-1}
\end{bmatrix}^T,
\end{align}
where $\tilde{\mathbf{p}}_k \in \mathbb{R}^{QP \times 1}$ represents the pressure at all point-like $QP$ transducers, for time $t = k \Delta t$. We can then define $\tilde{\mathbf{p}}^{SIR}_k \in \mathbb{R}^{Q \times 1}$ as 
\begin{align}\label{eq:3diii_indt}
\tilde{\mathbf{p}}^{SIR}_k = \boldsymbol{\gamma} \tilde{\mathbf{p}}_k,
\end{align}
where $\boldsymbol{\gamma} \in \mathbb{R}^{Q \times QP}$ describes the action in Eqn.~\eref{eq:3diii_SIRc}.
We can then construct a matrix $\boldsymbol{\Gamma}^{SIR} \in \mathbb{R}^{QK \times QPK}$ defined by
\begin{align}
\boldsymbol{\Gamma}^{SIR} \equiv \begin{bmatrix}
&\boldsymbol{\gamma} &\mathbf{0}_{Q\times QP} &\cdots &\mathbf{0}_{Q\times QP} \\
&\mathbf{0}_{Q\times QP} &\boldsymbol{\gamma} &\cdots &\mathbf{0}_{Q\times QP} \\
&\vdots &\vdots &\ddots &\vdots \\
&\mathbf{0}_{Q\times QP}  &\mathbf{0}_{Q\times QP} &\cdots &\boldsymbol{\gamma}\\
\end{bmatrix}
\end{align}
Given $\boldsymbol{\Gamma}^{SIR}$ we can then model the SIR effects of the transducer in the system matrix by applying the $\boldsymbol{\Gamma}^{SIR}$ after the application of the matrix $\mathbf{H}_{PS}$. Thus, the updated imaging equation is given by
\begin{align}
\tilde{\mathbf{p}}^{SIR} = \boldsymbol{\Gamma}^{SIR}\mathbf{H}_{PS} \boldsymbol{\theta}.
\end{align}

The EIR models the electrical response of the piezoelectric transducer. We assume that the transducer is a linear shift variant system with respect to the spatially averaged input time sequence. Hence, the output voltage signal of the transducer is the linear convolution between the EIR and the spatially averaged pressure time sequence~\cite{wang2011imaging}. We can model that mathematically as 
\begin{align}\label{eq:3diii_EIR}
\tilde{u}(\mathbf{r}_q^{\prime}, t) = h_e(t) *_t \tilde{p}^{SIR}(\mathbf{r}_q^{\prime}, t).
\end{align}
Hence, we can incorporate the action of the electrical impulse response in the discrete imaging model as 
\begin{align}\label{eq:3diii_Imageqn}
\tilde{\mathbf{u}} = \boldsymbol{\Gamma}^{EIR} \boldsymbol{\Gamma}^{SIR} \mathbf{H}_{PS} \boldsymbol{\theta},
\end{align}
where $\boldsymbol{\Gamma}^{EIR} \in \mathbb{R}^{QK \times QK}$ is a square matrix that can be constructed from the discretized numerical implementation of Eqn.~\ref{eq:3diii_EIR}~\cite{huang2013full}.
Thus the system matrix that numerically models the initial value problem defined in Eqns.~\eref{eq:2a_loss} and also the transducer impulse responses is given by
\begin{align}\label{eq:3d_iii_H}
\mathbf{H} = \boldsymbol{\Gamma}^{EIR} \boldsymbol{\Gamma}^{SIR} \mathbf{H}_{PS}.
\end{align} 

==> section7/section7a-old.tex <==
\subsection{Two-dimensional model applied to three dimensional systems}
\label{sec:7a}

\subsubsection{Use of 2D imaging model with 3D experimental systems}
\label{sec:7a_i}
Among many PACT experimental system designs, one practical and popular design employs a circular ring array with a number of focused transducer elements \cite{xia2014small,li2017single,xia2013enhancement,xi2012design,lou2014mouse}. 
During the imaging process, the ring array would take multiple ``snapshots" along the vertical (Z) direction, effectively forming a cylindrical measurement surface. 
And while reconstructing the PACT image, a 2D image in the X-Y plane would be reconstructed from each ``snapshot" according to a 2D wave propagation model, and stacked together along the Z direction to produce a 3D reconstructed volume of initial pressure distribution. 
By partition the entire measured dataset into ``2D" slices and reconstruct individual slices, this type of approach avoids the heavy computation burden related to directly consider and reconstruct a 3D volume.
However, there are two major limitations associated with this approach: 
First, even when recording with a focused 2D ring array, the acoustic wave propagation is still in a 3D space, resulting in a mismatch between the 2D model employed in the reconstruction process, and the 3D wave model that represents the true physics. 
Second, by individually reconstructing 2D slices, the integrity of the object along the Z direction is not considered.  
Therefore there remains a need to carefully investigate the accuracy of employing such a 2D model in this type of 3D cylindrical systems. 
In the following subsections, we will briefly present some preliminary insights and numerical results related to this issue, we hope these results can raise more concerns and interests from the general crowd. 

\subsubsection{Differences between 2D and 3D Green's functions}
\label{sec:7a_ii}
Similar issues have been studied in the geophysics community, where the tradeoff betweeen the accuracy of the wave propagation model  and computational burden is explored in the context of full waveform inversion (FWI)~\cite{auer2013critical}. 
Hence results from these studies can potentially provide valuable insights for us. 
In this subsection, we will review the difference between the 2D and 3D Green's functions and discuss some approaches that have been proposed to correct for the model mismatch between 3D and 2D wave propagation. 

The frequency domain solution to the 3D wave equation for a 3D point source in an unbounded, acoustically homogeneous medium can be expressed as \cite{aki2002quantitative,auer2013critical}
\begin{equation}
	\bar{G}^{3D}(\mathbf{r}, \omega) = \frac{1}{4 \pi |\mathbf{r}|} \exp \left( \frac{i \omega |\mathbf{r}| }{c} \right),
	\label{eq:7a_Green_3D}
\end{equation}
where $\mathbf{r}$ is the relative location of the receiver with respect to source, $\omega$ is the angular frequency, and $c$ is the speed of sound of the homogeneous medium. 

The frequency domain solution to the 2D wave equation under the same conditions is given by \cite{abramowitz1964handbook}
\begin{align}
	\bar{G}^{2D}(\mathbf{r}, \omega) &= \frac{i}{4} H_0^{(1)} \left( \frac{\omega |\mathbf{r}|}{c} \right)		\nonumber \\
		&\approx \frac{1}{2} \sqrt{\frac{c}{2\pi \omega |\mathbf{r}|}} \exp \left( \frac{i \omega |\mathbf{r}|}{c} \right) \exp \left( \frac{i \pi}{4} \right), 
	\label{eq:7a_Green_2D}
\end{align}
where $H_0^{(1)}$ is the Hankel function of the first kind and zero order, and when the distance $|\mathbf{r}|$ is relatively large compared to the wavelength $\frac{c}{\omega}$, the approximation is valid \cite{auer2013critical}. 

The difference between 3D and 2D wave propagation is in their varying amplitude
decay with distance. In the case of a 3D point source in a
homogeneous medium, energy spreads over the surface of a sphere,where the amplitude scales by $\frac{1}{|\mathbf{r}|}$. In the 2D case, energy spreads over
the surface of an expanding cylinder and the amplitude scale with $\frac{1}{\sqrt{|\mathbf{r}|}}$. 

Variety of authors have proposed using asymptotic point-source to line-source conversion filters to convert 3D data into 2D data~
\cite{yedlin2012uniform,bleistein2012mathematical}. The derivation
of the filter function is based on forming the ratio of the
acoustic 3D frequency-domain Green’s function defined in Eqn.~\eref{eq:7a_Green_3D} and
the asymptotic approximation of the acoustic 2D frequency-domain
Green’s function defined in Eqn.~\eref{eq:7a_Green_2D}. This yields the asymptotic
filter transfer function, with the Bleinstein filter function being the most widely used~\cite{bleistein2012mathematical}.

Conventionally, researchers correct for the model mismatch between data generated from 3D wave propagation and employing 2D wave propagation model in the reconstruction,  by transforming the recorded 3D field data to the approximate 2D equivalent by using such asymptotic filter algorithms. Such filters assume straight raypaths, a constant speed of sound medium, and far-field recordings. A crtitical study of 3D-2D transformation using asymptotic filters has been performed by propagating 3D wavefields, applying the filtering, and comparing the results of 2D FWI from filtered 3D wavefields~\cite{auer2013critical}. For an acoustically homogenous medium, the
FWI inversion results exhibited only marginal disparities between model
reconstructions from 2D data and filtered 3D data. Nevertheless, it was observed that, the asymptotic filters are less effective and we observe considerable waveform
misfits and artifacts in the FWI reconstructions when the medium is acoustically heterogenous. The source of these artifacts are due to the presence of 3D out of plane scatterers that can produce out of plane scattered signals which cannot be accounted for in the 2D reconstruction. Hence, experienced practitioners can help mitigate some of these out of plane scattering artifacts by carefully designing the elevational focusing properties of the transducers. 
\if 0 
\subsubsection{challenges with modelling ring-arrays, or other 2D-like systems, in 3D}
\subsubsection{Include numerical examples (Yang)}
\fi 


==> section7/section7e-old.tex <==
\subsection{Uncertainty quantification}

The image reconstruction problem in PACT is to estimate the finite dimensional representation of the 3D initial pressure distribution $\boldsymbol{\theta} \in \mathbb{R}^{N \times 1}$ from the recorded pressure data $\mathbf{u} \in \mathbb{R}^{QK \times 1}$. In this section, we shall review the inverse problem in 3D PACT from a 
Bayesian perspective~\cite{tarvainen2013bayesian,pulkkinen2014bayesian,koponen2014bayesian,tick2016image}. The discrete imaging model for 3D PACT in the presence of additive noise can be described as
\begin{align}
	\mathbf{u} = \mathbf{H} \boldsymbol{\theta} + \boldsymbol{\eta},
\end{align}
where $\mathbf{H} \in \mathbb{R}^{QK \times N}$ is the discrete forward PACT imaging model, while $\boldsymbol{\eta} \in \mathbb{R}^{QK \times 1}$ denotes the additive noise. In practice, the definition of $\mathbf{H}$ will vary based on the forward model employed to map the initial pressure distribution to the measured data. From a Bayesian framework, the image reconstruction problem can be interpreted as maximizing the posterior probability density $pr(\boldsymbol{\theta}| \mathbf{u})$. Hence, the maximum a posteriori estimate (MAP) is given by
\begin{align}
	\hat{\boldsymbol{\theta}}_{MAP} = \underset{\boldsymbol{\theta}}{\textnormal{argmin}}{\ - \log{pr(\boldsymbol{\theta}}| \mathbf{u})}.
\end{align}
From Baye's theorem we can interpret the MAP estimate as
\begin{align}\label{eq:7e_MAP}
	\hat{\boldsymbol{\theta}}_{MAP} = \underset{\boldsymbol{\theta}}{\textnormal{argmin}}{\Big[-\log pr(\mathbf{u} | \boldsymbol{\theta}) -  \log pr(\boldsymbol{\theta})\Big]},
\end{align}
where $pr(\mathbf{u} | \boldsymbol{\theta})$ is the likelihood density and $pr(\boldsymbol{\theta})$ is the prior probability density of the object model. If the noise $\eta$ and $\boldsymbol{\theta}$ are assumed to be mutually independent, the likelihood density is given by
\begin{align}
	pr (\mathbf{u}|\boldsymbol{\theta}) = pr_{\boldsymbol{\eta}} (\mathbf{u} - \mathbf{H}\boldsymbol{\theta}),
\end{align} 
where $pr_{\boldsymbol{\eta}}$ is the probability distribution of the noise $\boldsymbol{\eta}$. Let the initial pressure distribution $\boldsymbol{\theta}$ and the measurement noise $\boldsymbol{\eta}$ be modeled as Gaussian distributions. Thus we have $\boldsymbol{\theta} \sim \mathcal{N} (\boldsymbol{\mu}_{\theta}, \boldsymbol{\Gamma}_{\theta})$ and $\eta \sim \mathcal{N}(\boldsymbol{\mu}_{\eta}, \boldsymbol{\Gamma}_{\eta})$, where $\boldsymbol{\mu}_{\theta} \in \mathbb{R}^{N \times 1}$ and $\boldsymbol{\Gamma}_{\theta} \in \mathbb{R}^{N \times N}$ are the mean and covariance matrix of the prior distribution of the object model, while $\boldsymbol{\mu}_{\eta} \in \mathbb{R}^{QK \times 1}$ and $\boldsymbol{\Gamma}_{\eta} \in \mathbb{R}^{QK \times QK}$ is the mean and the covariance matrix of the noise. Given such assumption, the MAP estimate described in Eqn.~\eref{eq:7e_MAP} can be written as 
\begin{align}\label{eq:7e_MAPii}
	\hat{\boldsymbol{\theta}}_{MAP} = \underset{\boldsymbol{\theta}}{\textnormal{argmin}}{\Big[\frac{1}{2} ||\mathbf{L}_{\eta} (\mathbf{u} - \mathbf{H}\boldsymbol{\theta} - \boldsymbol{\mu}_{\eta})||_2^2 + \frac{1}{2}||\mathbf{L}_{\theta}(\boldsymbol{\theta} - \boldsymbol{\mu}_{\theta})||_2^2\Big]},
\end{align}
where $\mathbf{L}_{\eta} \in \mathbb{R}^{QK \times QK}$ and $\mathbf{L}_{\theta} \in \mathbb{R}^{N \times N}$ are the Cholesky decompositions of the inverse covariance matrices of the noise and the object prior respectively, i.e. $\mathbf{L}_{\eta}^{T}\mathbf{L}_{\eta} = \boldsymbol{\Gamma}_{\eta}^{-1}$ and $\mathbf{L}_{\theta}^{T}\mathbf{L}_{\theta} = \boldsymbol{\Gamma}_{\theta}^{-1}$. Furthermore, when the imaging model is linear, the object prior and the noise model is gaussian, the  posterior distribution is also gaussian, i.e. $pr(\boldsymbol{\theta}|\mathbf{u}) \sim \mathcal{N}(\boldsymbol{\mu}_{\theta|\tilde{u}}, \boldsymbol{\Gamma}_{{\theta} | \tilde{u}})$. The mean and the covariance matrix of the posterior distribution is given by
\begin{align}
	\mu_{\theta|\tilde{u}} &= \Big(\mathbf{H}^{\dagger}\boldsymbol{\Gamma}_{\eta}^{-1}\mathbf{H} + \boldsymbol{\Gamma}_{\theta}^{-1}\Big)^{-1} \Big(\mathbf{H}^{\dagger}\boldsymbol{\Gamma}_{\eta}^{-1}(\mathbf{u} - \boldsymbol{\mu}_{\eta}) + \boldsymbol{\Gamma}_{\theta}^{-1}\boldsymbol{\mu}_{\theta}\Big) \nonumber \\
	\boldsymbol{\Gamma}_{\theta | \tilde{u}} &= \Big(\mathbf{H}^{\dagger}\boldsymbol{\Gamma}_{\eta}^{-1}\mathbf{H} + \boldsymbol{\Gamma}_{\theta}^{-1}\Big)^{-1}.
\end{align}
The MAP estimate described in Eqn.~\ref{eq:7e_MAPii} is a point estimate of the posterior distribution. For a purely Gaussian case that we have considered, the MAP estimate is the mean of the posterior distribution, i.e. $\hat{\boldsymbol{\theta}}_{MAP} = \boldsymbol{\mu}_{\theta | \tilde{u}}$. In addtion we can also observe from Eqn.~\eref{eq:7e_MAPii}, that the MAP estimate resembles the solution of a minimization problem for a generalized penalized least squares method described in Eqn.~\eref{eq:4c_ii_PLS}. 

Note, as part of computing the posterior distribution $pr(\boldsymbol{\theta}|\mathbf{u})$, we can information about the variance of the MAP estimate. The information regarding the variance of the reconstructed image directly reveals the reliability of different regions in the reconstruction image. It can also serve as a metric to quantify imaging system performance, and therefore can help guide system design~\cite{huesman1984new,sijbers1999parameter}.
The uncertainty distribution of the reconstructed MAP estimates can be computed using the marginal density of the posterior distribution. Since, we have assumed that the posterior density is a Gaussian, the marginal density for the $k$th element of $\boldsymbol{\theta}$ is defined as 
\begin{align}
	\hat{\boldsymbol{\theta}}_{MAP} \sim \mathcal{N}([\boldsymbol{\mu}_{\theta| \tilde{u}}]_k, [\boldsymbol{\Gamma}_{\theta | \tilde{u}}]_{kk}),
\end{align}
where $[\boldsymbol{\mu}_{\theta| \tilde{u}}]_k$  and $[\boldsymbol{\Gamma}_{\theta | \tilde{u}}]_{kk}$ are the $k$th element of $\boldsymbol{\mu}_{\theta| \tilde{u}}$ and the $k$th diagnol element of $\boldsymbol{\Gamma}_{\theta | \tilde{u}}$, respectively. Hence, a spatial map of $[\boldsymbol{\Gamma}_{\theta | \tilde{u}}]_{kk}$ for all the elements of the MAP estimate, gives us a measure of the uncertainty of the reconstruction. 

\subsubsection{Prior model}
As mentioned previously, depending on the choice of the noise model and the object prior model the MAP estimate of Eqn.~\ref{eq:7e_MAPii} can be equivalent to solving the penalized least squares estimate in Eqn.~\ref{eq:4c_ii_PLS}. For PACT reconstruction, previous works have commonly employed white noise prior and the Mat\'ern prior. The choice of the white noise prior object model is equivalent to solving the penalized least squares problem in Eqn.~\ref{eq:4c_ii_PLS} with Tikhonov regularization. The white noise prior assumes that the estimated parameters/pixels have no spatial correlation. The Mat\'ern prior, on the otherhand, supports correlation between pixels. The covariance matrix of the Mat\'ern prior is defined as
\begin{align}
	[\boldsymbol{\Gamma}_{\theta}]_{ij} = \sigma_m^2 \frac{2^{1- \nu}}{G(\nu)}\Big(\frac{\sqrt{2 \nu}||r_i - r_j||}{l}\Big)^{\nu} K_{\nu} \Big(\frac{\sqrt{2\nu}||r_i - r_j||}{l}\Big),
\end{align}
where $i$ and $j$ are the element indices, $r_i$ and $r_j$ are the corresponding pixel locations, $\sigma_m^2$ is the variance, $\nu > 0$ is the smoothness parameter, $l$ is the length scale, $G$ is the gamma-function, and $K_{\nu}$ is the modified Bessel function of the second kind of order $\nu$~\cite{rasmussen2004gaussian}. With the Mat\'ern object prior, we can promote distributions that can be homogeneous locally with sharp changes between different areas depending on the scale $l$. Such a prior is assumed to be suitable for modeling distributions of blood vessels in photoacoustic imaging~\cite{tick2016image}. 


==> section7/section7e.tex <==
\subsection{Uncertainty quantification}

Uncertainity quantification (UQ) is the end-to-end study of the impact of all forms of error and uncertainty in the models arising in the applications. The questions considered range from fundamental, mathematical, and statistical questions to practical questions of computational accuracy and cost [1]. Research into these questions takes place at ZIB in the Uncertainty Quantification group, and finds applications in other working groups such as Computational Medicine, Computational Molecular Design, and Visualization.

Roughly speaking, UQ divides into two major branches, forward and inverse problems. In the forward propagation of uncertainty, we have a known model F for a system of interest. We model its inputs X as a random variable and wish to understand the output random variable Y = F(X), sometimes denoted Y|X, read as “Y given X.” There is a substantial overlap between this area and sensitivity analysis, since the random variations in X probe the sensitivity of the forward model F to changes of its inputs. In the other major branch of UQ, inverse problems, F is still the forward model, but now Y denotes some observed data, and we wish to infer inputs X so that F(X) = Y; that is, we want not Y|X but X|Y. Here, there is substantial overlap with statistical inference and with imaging and data analysis. Inverse problems typically have no solutions in the literal sense, because our models F are only approximate, there is no X for which F(X) agrees exactly with the observed data Y. Therefore, it becomes necessary to relax the notion of a solution, and often also to incorporate prior or expert knowledge on what a “good” solution X might be. In recent years, the Bayesian perspective on inverse problems has received much attention, because it is powerful and flexible enough to meet these requirements, and because increased computational power makes the Bayesian approach more feasible than in decades past [2].  In the Bayesian perspective, we again regard X and Y as random variables and encode our prior expert knowledge about X into a prior probability distribution p(X), which we condition with respect to Y using Bayes’ rule 

p(X|Y) = p(Y|X) p(X) / p(Y)

to produce a so-called posterior distribution for X|Y, which is the mathematical representation of all knowledge/uncertainty about X, given the observed data Y and the expert knowledge encoded in the prior p(X). However, the posterior p(X|Y) is typically a very complicated distribution on a large space (the space of unknown Xs that we are trying to infer), so there are major mathematical and computational challenges in implementing this fully Bayesian approach, and in producing appropriate simplifications for end users.



\if 0
The image reconstruction problem in PACT is to estimate the finite dimensional representation of the 3D initial pressure distribution $\boldsymbol{\theta} \in \mathbb{R}^{N \times 1}$ from the recorded pressure data $\mathbf{u} \in \mathbb{R}^{QK \times 1}$. In this section, we shall review the inverse problem in 3D PACT from a 
Bayesian perspective~\cite{tarvainen2013bayesian,pulkkinen2014bayesian,koponen2014bayesian,tick2016image}. The discrete imaging model for 3D PACT in the presence of additive noise can be described as
\begin{align}
	\mathbf{u} = \mathbf{H} \boldsymbol{\theta} + \boldsymbol{\eta},
\end{align}
where $\mathbf{H} \in \mathbb{R}^{QK \times N}$ is the discrete forward PACT imaging model, while $\boldsymbol{\eta} \in \mathbb{R}^{QK \times 1}$ denotes the additive noise. In practice, the definition of $\mathbf{H}$ will vary based on the forward model employed to map the initial pressure distribution to the measured data. From a Bayesian framework, the image reconstruction problem can be interpreted as maximizing the posterior probability density $pr(\boldsymbol{\theta}| \mathbf{u})$. Hence, the maximum a posteriori estimate (MAP) is given by
\begin{align}
	\hat{\boldsymbol{\theta}}_{MAP} = \underset{\boldsymbol{\theta}}{\textnormal{argmin}}{\ - \log{pr(\boldsymbol{\theta}}| \mathbf{u})}.
\end{align}
From Baye's theorem we can interpret the MAP estimate as
\begin{align}\label{eq:7e_MAP}
	\hat{\boldsymbol{\theta}}_{MAP} = \underset{\boldsymbol{\theta}}{\textnormal{argmin}}{\Big[-\log pr(\mathbf{u} | \boldsymbol{\theta}) -  \log pr(\boldsymbol{\theta})\Big]},
\end{align}
where $pr(\mathbf{u} | \boldsymbol{\theta})$ is the likelihood density and $pr(\boldsymbol{\theta})$ is the prior probability density of the object model. If the noise $\eta$ and $\boldsymbol{\theta}$ are assumed to be mutually independent, the likelihood density is given by
\begin{align}
	pr (\mathbf{u}|\boldsymbol{\theta}) = pr_{\boldsymbol{\eta}} (\mathbf{u} - \mathbf{H}\boldsymbol{\theta}),
\end{align} 
where $pr_{\boldsymbol{\eta}}$ is the probability distribution of the noise $\boldsymbol{\eta}$. Let the initial pressure distribution $\boldsymbol{\theta}$ and the measurement noise $\boldsymbol{\eta}$ be modeled as Gaussian distributions. Thus we have $\boldsymbol{\theta} \sim \mathcal{N} (\boldsymbol{\mu}_{\theta}, \boldsymbol{\Gamma}_{\theta})$ and $\eta \sim \mathcal{N}(\boldsymbol{\mu}_{\eta}, \boldsymbol{\Gamma}_{\eta})$, where $\boldsymbol{\mu}_{\theta} \in \mathbb{R}^{N \times 1}$ and $\boldsymbol{\Gamma}_{\theta} \in \mathbb{R}^{N \times N}$ are the mean and covariance matrix of the prior distribution of the object model, while $\boldsymbol{\mu}_{\eta} \in \mathbb{R}^{QK \times 1}$ and $\boldsymbol{\Gamma}_{\eta} \in \mathbb{R}^{QK \times QK}$ is the mean and the covariance matrix of the noise. Given such assumption, the MAP estimate described in Eqn.~\eref{eq:7e_MAP} can be written as 
\begin{align}\label{eq:7e_MAPii}
	\hat{\boldsymbol{\theta}}_{MAP} = \underset{\boldsymbol{\theta}}{\textnormal{argmin}}{\Big[\frac{1}{2} ||\mathbf{L}_{\eta} (\mathbf{u} - \mathbf{H}\boldsymbol{\theta} - \boldsymbol{\mu}_{\eta})||_2^2 + \frac{1}{2}||\mathbf{L}_{\theta}(\boldsymbol{\theta} - \boldsymbol{\mu}_{\theta})||_2^2\Big]},
\end{align}
where $\mathbf{L}_{\eta} \in \mathbb{R}^{QK \times QK}$ and $\mathbf{L}_{\theta} \in \mathbb{R}^{N \times N}$ are the Cholesky decompositions of the inverse covariance matrices of the noise and the object prior respectively, i.e. $\mathbf{L}_{\eta}^{T}\mathbf{L}_{\eta} = \boldsymbol{\Gamma}_{\eta}^{-1}$ and $\mathbf{L}_{\theta}^{T}\mathbf{L}_{\theta} = \boldsymbol{\Gamma}_{\theta}^{-1}$. Furthermore, when the imaging model is linear, the object prior and the noise model is gaussian, the  posterior distribution is also gaussian, i.e. $pr(\boldsymbol{\theta}|\mathbf{u}) \sim \mathcal{N}(\boldsymbol{\mu}_{\theta|\tilde{u}}, \boldsymbol{\Gamma}_{{\theta} | \tilde{u}})$. The mean and the covariance matrix of the posterior distribution is given by
\begin{align}
	\mu_{\theta|\tilde{u}} &= \Big(\mathbf{H}^{\dagger}\boldsymbol{\Gamma}_{\eta}^{-1}\mathbf{H} + \boldsymbol{\Gamma}_{\theta}^{-1}\Big)^{-1} \Big(\mathbf{H}^{\dagger}\boldsymbol{\Gamma}_{\eta}^{-1}(\mathbf{u} - \boldsymbol{\mu}_{\eta}) + \boldsymbol{\Gamma}_{\theta}^{-1}\boldsymbol{\mu}_{\theta}\Big) \nonumber \\
	\boldsymbol{\Gamma}_{\theta | \tilde{u}} &= \Big(\mathbf{H}^{\dagger}\boldsymbol{\Gamma}_{\eta}^{-1}\mathbf{H} + \boldsymbol{\Gamma}_{\theta}^{-1}\Big)^{-1}.
\end{align}
The MAP estimate described in Eqn.~\ref{eq:7e_MAPii} is a point estimate of the posterior distribution. For a purely Gaussian case that we have considered, the MAP estimate is the mean of the posterior distribution, i.e. $\hat{\boldsymbol{\theta}}_{MAP} = \boldsymbol{\mu}_{\theta | \tilde{u}}$. In addtion we can also observe from Eqn.~\eref{eq:7e_MAPii}, that the MAP estimate resembles the solution of a minimization problem for a generalized penalized least squares method described in Eqn.~\eref{eq:4c_ii_PLS}. 

Note, as part of computing the posterior distribution $pr(\boldsymbol{\theta}|\mathbf{u})$, we can information about the variance of the MAP estimate. The information regarding the variance of the reconstructed image directly reveals the reliability of different regions in the reconstruction image. It can also serve as a metric to quantify imaging system performance, and therefore can help guide system design~\cite{huesman1984new,sijbers1999parameter}.
The uncertainty distribution of the reconstructed MAP estimates can be computed using the marginal density of the posterior distribution. Since, we have assumed that the posterior density is a Gaussian, the marginal density for the $k$th element of $\boldsymbol{\theta}$ is defined as 
\begin{align}
	\hat{\boldsymbol{\theta}}_{MAP} \sim \mathcal{N}([\boldsymbol{\mu}_{\theta| \tilde{u}}]_k, [\boldsymbol{\Gamma}_{\theta | \tilde{u}}]_{kk}),
\end{align}
where $[\boldsymbol{\mu}_{\theta| \tilde{u}}]_k$  and $[\boldsymbol{\Gamma}_{\theta | \tilde{u}}]_{kk}$ are the $k$th element of $\boldsymbol{\mu}_{\theta| \tilde{u}}$ and the $k$th diagnol element of $\boldsymbol{\Gamma}_{\theta | \tilde{u}}$, respectively. Hence, a spatial map of $[\boldsymbol{\Gamma}_{\theta | \tilde{u}}]_{kk}$ for all the elements of the MAP estimate, gives us a measure of the uncertainty of the reconstruction. 

\subsubsection{Prior model}
As mentioned previously, depending on the choice of the noise model and the object prior model the MAP estimate of Eqn.~\ref{eq:7e_MAPii} can be equivalent to solving the penalized least squares estimate in Eqn.~\ref{eq:4c_ii_PLS}. For PACT reconstruction, previous works have commonly employed white noise prior and the Mat\'ern prior. The choice of the white noise prior object model is equivalent to solving the penalized least squares problem in Eqn.~\ref{eq:4c_ii_PLS} with Tikhonov regularization. The white noise prior assumes that the estimated parameters/pixels have no spatial correlation. The Mat\'ern prior, on the otherhand, supports correlation between pixels. The covariance matrix of the Mat\'ern prior is defined as
\begin{align}
	[\boldsymbol{\Gamma}_{\theta}]_{ij} = \sigma_m^2 \frac{2^{1- \nu}}{G(\nu)}\Big(\frac{\sqrt{2 \nu}||r_i - r_j||}{l}\Big)^{\nu} K_{\nu} \Big(\frac{\sqrt{2\nu}||r_i - r_j||}{l}\Big),
\end{align}
where $i$ and $j$ are the element indices, $r_i$ and $r_j$ are the corresponding pixel locations, $\sigma_m^2$ is the variance, $\nu > 0$ is the smoothness parameter, $l$ is the length scale, $G$ is the gamma-function, and $K_{\nu}$ is the modified Bessel function of the second kind of order $\nu$~\cite{rasmussen2004gaussian}. With the Mat\'ern object prior, we can promote distributions that can be homogeneous locally with sharp changes between different areas depending on the scale $l$. Such a prior is assumed to be suitable for modeling distributions of blood vessels in photoacoustic imaging~\cite{tick2016image}. 
\fi

